Error estimates for vector field interpolation based on generalized matrix-valued kernels

Matrix-valued kernels provide a flexible framework for approximating vector fields from scattered data, especially when structural constraints such as divergence-free or curl-free conditions must be preserved. Classical potential-based constructions enforce these constraints naturally, but they typically require the generating scalar function to possess relatively high smoothness. We develop an operator-based framework for constructing div-free and curl-free matrix-valued kernels using integral and differential operators, which substantially relaxes the regularity requirements of the potential approach. Using dimension-walking techniques, we show that the resulting native spaces are norm-equivalent to appropriate vector-valued Sobolev spaces. Another main contribution of the paper is a sharp error analysis for the corresponding kernel matrix-valued interpolation problem. We derive direct Sobolev error estimates that allow fractional regularity of the target field, and we establish Bernstein-type inequalities for the associated kernel trial spaces. These results lead to a complete inverse theorem. We also investigate stability by proving lower bounds for the smallest eigenvalues of the interpolation matrices. Numerical experiments are included to verify the theoretical results.

==> macro.tex <==
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}
\newcommand{\green}[1]{{\color{green} #1}}
\newcommand{\dgreen}[1]{{\color[RGB]{0,100,0} #1}}
\newcommand{\magenta}[1]{{\color{magenta} #1}}

\definecolor{g1}{HTML}{2da02d}
\definecolor{r1}{HTML}{d62728}
\definecolor{b1}{HTML}{2178b5}

\definecolor{Cerulean}{HTML}{00A2E3}
\definecolor{JungleGreen}{HTML}{00A99A}
\definecolor{Orange}{HTML}{F58137}

\numberwithin{equation}{section}

\allowdisplaybreaks[3]




\newcommand*{\QEDB}{\hfill\ensuremath{\square}}%

% mathbb
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
% mathcal
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\rot}{\text{rot}}

\newcommand{\CK}{\mathcal{C}_K}
\newcommand{\bla}{{\bld \lambda}}
\newcommand{\ba}{\bm a}
\newcommand{\eps}{\varepsilon}
\newcommand{\Ome}{{\Omega}}
\newcommand{\ome}{{\omega}}
\newcommand{\p}{{\partial}}
\newcommand{\Del}{{\Delta}}
\newcommand{\nab}{\nabla}
\newcommand{\vare}{\bm{\varepsilon}}
\newcommand{\nonum}{\nonumber}
\renewcommand{\(}{\bigl(} 
\renewcommand{\)}{\bigr)}
\newcommand{\lt}{{L^2(\Ome)}}
\newcommand {\ho}{{H^1(\Ome)}}
\newcommand{\htw}{{H^2(\Ome)}}
\newcommand{\hl}{{H^\ell(\Ome)}}
\newcommand{\htwt}{{H^2(T)}}
\newcommand{\lte}{{L^2(e)}}
\newcommand{\bl}{\bigl\langle}
\newcommand{\br}{\bigr\rangle}
\newcommand{\Bl}{\Bigl\langle}
\newcommand{\Br}{\Bigr\rangle}
\newcommand{\mce}{\mathcal{E}_h}
\newcommand{\mcei}{\mce^i}
\newcommand{\mceb}{\mce^b}
\newcommand{\mct}{\mathcal{T}_h}
\newcommand{\mcc}{\mathcal{C}}
\newcommand{\avg}[1]{\bigl\{\hspace{-0.045in}\bigl\{#1\bigr\}\hspace{-0.045in}\bigr\}}
\newcommand{\bavg}[1]{\left\{\hspace{-0.065in}\left\{#1\right\}\hspace{-0.065in}\right\}}
\newcommand{\jump}[1]{\left[\hspace{-0.025in}\left[#1\right]\hspace{-0.025in}\right]}
\newcommand{\tbar}[1]{\left|\hspace{-0.015in}\left|\hspace{-0.015in}\left|#1\right|\hspace{-0.015in}\right|\hspace{-0.015in}\right|}
\newcommand{\vh}{V_h}
\newcommand{\ueh}{u^\alpha_h}
\newcommand{\uh}{u_h}
\newcommand{\ue}{u^\alpha}
\newcommand{\cof}{{\rm cof}}
\newcommand{\uc}{u_{c,h}}
\newcommand{\les}{\lesssim}
\newcommand{\ges}{\gtrsim}
\newcommand{\Ph}{\mathcal{P}_h}
\newcommand{\mcf}{{e}}
\newcommand{\ez}{e_z}
\newcommand{\curl}{{\ensuremath\mathop{\mathrm{curl}\,}}}
%\newcommand{\grad}{{\ensuremath\mathop{\mathrm{\bf grad}\,}}}
\newcommand{\dive}{{\ensuremath\mathop{\mathrm{div}\,}}}
\newcommand{\Div}{{\rm div}\,}
\newcommand{\bcurl}{{\bld{\curl}}}
\newcommand{\bG}{\bld{G}}
\newcommand{\RRR}{\mathbb{R}}
\newcommand{\ip}[1]{\big\langle {#1} \big\rangle}
\newcommand{\ipb}[1]{(\!\!\!( \,{{#1}}\, )\!\!\!)_b}
\newcommand{\pol}{\EuScript{P}}
\newcommand{\bpol}{\boldsymbol{\pol}}
\newcommand{\bld}[1]{\boldsymbol{#1}}
\newcommand{\bt}{\bld{t}}
\newcommand{\bchi}{\bld{\chi}}
\newcommand{\bkappa}{\bld{\kappa}}
\newcommand{\bI}{\bld{I}}
\newcommand{\bA}{\bld{A}}
\newcommand{\bb}{\bld{b}}
\newcommand{\ff}{{\bld{f}}}
\newcommand{\bY}{\bld{Y}}
\newcommand{\bv}{\bld{v}}
\newcommand{\bw}{\bld{w}}
\newcommand{\dbw}{\dot{\bld{w}}}
\newcommand{\bs}{\bld{s}}
\newcommand{\bp}{\bld{p}}
\newcommand{\bn}{\bld{n}}
\newcommand{\bu}{\bld{u}}
\newcommand{\tbu}{\bld{\tilde{u}}}
\newcommand{\bJ}{\bld{J}}
\newcommand{\bU}{\bld{U}}
\newcommand{\tsig}{\tilde{\sigma}_f}
\newcommand{\bE}{\bld{E}}
\newcommand{\bW}{\bld{W}}
\newcommand{\bV}{\bld{V}}
\newcommand{\bR}{\bld{R}}
\newcommand{\bS}{\bld{S}}
\newcommand{\bM}{\bld{M}}
\newcommand{\bD}{\bld{A}}
\newcommand{\btheta}{\bld{\theta}}
\newcommand{\bDi}{\mathcal{D}}
\newcommand{\bN}{\bld{N}}
\newcommand{\bq}{\bld{q}}
\newcommand{\blam}{\bld{\lambda}}
\newcommand{\bPi}{\bld{\Pi}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bZ}{\bld{Z}}
\newcommand{\brho}{\bld{\rho}}
\newcommand{\bzeta}{\bld{\zeta}}
\newcommand{\bsigma}{\bld{\sigma}}
\newcommand{\bH}{\bld{H}}
\newcommand{\bQ}{\bld{Q}}
\newcommand{\by}{\bld{y}}
\newcommand{\bmu}{{\bld{\mu}}}
\newcommand{\bgamma}{{\bld{\gamma}}}
\newcommand{\bx}{\bld{x}}
\newcommand{\bC}{\bld{C}}
\newcommand{\bL}{\bld{L}}
\newcommand{\bphi}{\bm \phi}
\newcommand{\Dim}{{\rm dim}\,}
\newcommand{\dK}{\partial K}
\newcommand{\Om}{\Omega}
\newcommand{\dOh}{{\partial \Omega_h}}
\newcommand{\Oh}{{\Omega_h}}
\newcommand{\bX}{{\bm X}}
\newcommand{\btau}{{\bm \tau}}
\newcommand{\balpha}{{\bm \alpha}}
\newcommand{\bbeta}{{\bm \beta}}
\newcommand{\bfeta}{{\bm \eta}}
\newcommand{\bff}{{\bm f}}
\newcommand{\dbfeta}{\dot{\bm \eta}}
\newcommand{\bPhi}{{\bm \Phi}}
\newcommand{\bvarphi}{\bm \varphi}
%\newcommand{\bpsi}{\bm \psi}
\newcommand{\bpsi}{\bm \psi}
\newcommand{\Dt}{\Delta t}
\newcommand{\uu}{\mathsf{u}}
\newcommand{\ww}{\mathsf{w}}
\newcommand{\qq}{\mathsf{q}}
\newcommand{\lla}{\mathsf{l}}
\newcommand{\Ll}{\mathcal{L}}
\newcommand{\Lla}{\Lambda}

\newcommand{\dd}{\delta}

\newcommand{\tg}{\tilde{g}}

\newcommand{\be}{\bm e}
\newcommand{\bc}{\bm c}
\newcommand{\bUpsilon}{\bm \Upsilon}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\MV}{\bV^{\rm MB}}
\newcommand{\BR}{\bV^{\rm BR}}

\newcommand{\mV}{\mathring{V}}
\newcommand{\calT}{\mathcal{T}}

\newcommand{\UU}{\mathcal{U}}
\newcommand{\tUU}{\tilde{\mathcal{U}}}

%%%%%%%%

\newcommand{\ef}{e_{f}}
\newcommand{\es}{e_{s}}
\newcommand{\eeta}{\bld{e}_{\eta}}
\newcommand{\edeta}{\dot{\bld{e}}_{\eta}}
\newcommand{\teu}{\tilde{\bld{e}}_{u}}
\newcommand{\tef}{\tilde{e}_{f}}
\newcommand{\pdt}{\partial_{\Delta t}}
\newcommand{\pt}{\partial_{t}}
\newcommand{\dt}{\Delta t}
\newcommand{\Z}{\mathsf{Z}}
\newcommand{\Ss}{\mathsf{S}}
\newcommand{\J}{\mathsf{J}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\revj}[1]{{\color{red}#1}}

\newcommand{\MJN}[1]{{\color{blue}#1}}
\newcommand{\TODO}[1]{{\color{magenta}TODO #1}}

\newcommand{\bPsi}{{\bm \Psi}}
\newcommand{\calE}{\mathcal{E}}


\def\eref#1{{\rm (\ref{#1})}}
\def\fref#1{{Fig.~\ref{#1}}}
\def\sref#1{{Sect.~\ref{#1}}}
\def\tref#1{{Tab.~\ref{#1}}}
\def\aref#1{{Alg.~\ref{#1}}}
\def\lref#1{{Lem.~\ref{#1}}}

\def\pn{\par\noindent}
\def\pf{\pn\textbf{Proof.}\enspace\ignorespaces}%
\def\qed{~\relax\ifmmode\hskip2em \Box
 \else\unskip\nobreak\hskip1em \hfill$\Box$
 \fi \newline}

% below are setup for easy notations update
\newmuskip\pFqmuskip

\newcommand*\pFq[6][8]{%
  \begingroup % only local assignments
  \pFqmuskip=#1mu\relax
  \mathchardef\normalcomma=\mathcode`,
  % make the comma math active
  \mathcode`\,=\string"8000
  % and define it to be \pFqcomma
  \begingroup\lccode`\~=`\,
  \lowercase{\endgroup\let~}\pFqcomma
  % typeset the formula
  {}_{#2}F_{#3}{\left(\genfrac..{0pt}{}{#4}{#5};#6\right)}%
  \endgroup
}
\newcommand{\pFqcomma}{{\normalcomma}\mskip\pFqmuskip}

\newcommand{\hgeom}[2]{\,{}_{#1\!}F_{#2}}


% speical character
\def\d{\mathrm{d}}
\def\dmu{\d\mu(x)}
\def\i{\mathrm{i}}


\def\varphim{\varphi_{2m+2}}
\def\I{\mathcal{I}}
\def\ftil{\widetilde{f}}
\def\fhat{\widehat{f}}
\def\phat{\widehat{\psi}}
\def\Phat{\widehat{\Psi}}
\def\chat{\widehat{\chi_N}}
\def\sphHarm{\mathcal{Y}_{\ell,k}}


\def\Pro{\Phi_{\rho}}
\def\Pmro{\Phi_{\rho}^m}
\def\pmro{\phi_{\rho}^m}
\def\hatPmr{\widehat{\Phi}_{\rho}^m}
\def\IntSph{\int_{\bbS^d}}
\def\ConvPhi{\mathcal{C}_{\varphi_{\rho}}}
\def\Nro{N_{\rho}}
\def\tchie{\chi_{\eta}}
\def\tomge{\omega_{\eta}}
\def\QuadSet{\mathcal{Q}_{X}}
\def\scaleKer{\varphi_{\rho}}

\def\sphHarm{\mathcal{Y}_{\ell k}}
\def\Omgk{\omega_k}
\def\Ix{\mathcal{I}_X}
\def\Qi{Q_{X,\rho}}
\def\QiE{\cQ_{\scaleKer}^{q,\bm{\varepsilon}}}
\def\Hsig{H^{\sigma}}
\def\Htau{H^{\tau}}
\def\Hatf{\widehat{f}_{\ell,k}}
\def\HatKer{\widehat{\scaleKer}(\ell)}
\def\HatQi{\widehat{\cQ_{\scaleKer}^q f}_{\ell,k}}
\def\fInf{\|f\|_{L_{\infty}}}
\def\fHsig{\|f\|_{\Hsig}}
\def\gInf{\|g\|_{L_{\infty}}}
\def\gHsig{\|g\|_{\Hsig}}

\def\Delro{\Delta_{\rho}}
\def\Delh{\Delta_{h}}

%% numerical solution
\def\tilU{\widetilde{U}}
\def\tilu{\tilde{\bu}}
\def\halfn{{n+\frac{1}{2}}}
\def\uhalfn{u^{n+\frac{1}{2}}}
\def\Ehalfn{\cE[\uhalfn]}
\def\Etilun{\cE[\tilu^n]}
\def\EtilU{\cE{[\tilU^n]}}
\def\Ghalfun{\G(\uhalfn)}
\def\Gtilun{\G(\tilu^n)}
\def\Ghtilun{\G(\tilu^n)}



\def\Sumlk{\sum_{\ell=0}^{\infty}\sum_{k=0}^{Z(d,\ell)}}
